xLSTM: Extended Long Short-Term Memory

In the 1990s, the constant error carousel and gating were introduced as the central ideas of the Long Short-Term Memory (LSTM). Since then, LSTMs have stood the test of time and contributed to numerous deep learning success stories, in particular they constituted the first Large Language Models (LLMs). However, the advent of the Transformer technology with parallelizable self-attention at its core marked the dawn of a new era, outpacing LSTMs at scale. We now raise a simple question: How far do we get in language modeling when scaling LSTMs to billions of parameters, leveraging the latest techniques from modern LLMs, but mitigating known limitations of LSTMs? Firstly, we introduce exponential gating with appropriate normalization and stabilization techniques. Secondly, we modify the LSTM memory structure, obtaining: (i) sLSTM with a scalar memory, a scalar update, and new memory mixing, (ii) mLSTM that is fully parallelizable with a matrix memory and a covariance update rule. Integrating these LSTM extensions into residual block backbones yields xLSTM blocks that are then residually stacked into xLSTM architectures. Exponential gating and modified memory structures boost xLSTM capabilities to perform favorably when compared to state-of-the-art Transformers and State Space Models, both in performance and scaling.

==> commands/colors.tex <==


\definecolor{col-xlstm}{HTML}{}
\definecolor{col-mlstm}{HTML}{}
\definecolor{col-slstm}{HTML}{}
\definecolor{col-mamba-wt}{HTML}{}
\definecolor{col-mamba-nwt}{HTML}{}
\definecolor{col-lama}{HTML}{}
\definecolor{col-rwkv4}{HTML}{}
\definecolor{col-rwkv5}{HTML}{}
\definecolor{col-rwkv6}{HTML}{}
\definecolor{col-lstm}{HTML}{}
\definecolor{col-lstmmix}{HTML}{}
\definecolor{col-lru}{HTML}{}
\definecolor{col-retention}{HTML}{}
\definecolor{col-h3}{HTML}{}
\definecolor{col-hyena}{HTML}{}


==> commands/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/comp_spaj15b_model_benchmark_twocol.tex <==
\begin{minipage}{0.45\textwidth}

\begin{tabular}{lcr}
    \toprule
    Model               & \thead{\#Params                              \\ M} & \thead{SlimPajama \\ (15B) ppl $\downarrow$}\\
    \midrule
    Hyena               & 435             & 17.59                      \\
    RWKV-4              & 430             & 15.62          \\
    RWKV-5              & 456             & \underline{14.25}                      \\
    RWKV-6              & 442             & 15.03                      \\
    RetNet              & 431             & 16.23                      \\
    % HGRN                & 411             & 21.83                      \\
    GLA                 & 412             & 16.15                      \\
    HGRN2               & 411             & 14.32                      \\
    \bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{0.45\textwidth}
\vspace{-0.05cm}
\begin{tabular}{lcr}
    \toprule
    Model               & \thead{\#Params                              \\ M} & \thead{SlimPajama \\ (15B) ppl $\downarrow$}\\
    \midrule
    GPT-3               & 356             & 14.26                      \\
    Llama               & 407             & \underline{14.25}          \\
    % \midrule
    % LSTM-block          & 506             & \underline{26.07}          \\
    \midrule
    H3                  & 420             & 18.23                      \\
    Mamba               & 423             & \underline{13.70}          \\
    \midrule
    % \textbf{xLSTM[0:1]} & 402             & 18.08                      \\
    \textbf{xLSTM[1:0]} & 409             & \underline{\textbf{13.43}} \\
    \textbf{xLSTM[7:1]} & 408             & 13.48                      \\
    \bottomrule
\end{tabular}
\end{minipage}


==> tables/lra_hyperparameters.tex <==
\begin{table}
    \begin{adjustbox}{width=1.0\textwidth}
    \begin{tabular}[htp]{m{1.5cm}m{2cm}m{1.6cm}m{1.85cm}p{1cm}m{1.4cm}m{1.7cm}m{1cm}}
    \toprule
         \multirow{2}{1cm}{\textbf{Task}} & \multirow{2}{2cm}{\textbf{Model}} & \multirow{2}{1.6cm}{\textbf{Number of blocks}} & \multirow{2}{1.8cm}{\textbf{Embedding dimension}} & \multirow{2}{1cm}{\textbf{Batch size}} &  \multirow{2}{1.4cm}{\textbf{Number of steps}} &  \multirow{2}{1.8cm}{\textbf{LR scheduler}} &  \multirow{2}{1.6cm}{\textbf{LR}} \\
         &  &  &  &  &  &  & \\
    \midrule
        \multirow{9}{*}{Retrieval} & Transformer & \multirow{9}{*}{6} & \multirow{9}{*}{128} & \multirow{9}{*}{64} & \multirow{9}{*}{100K} & WCAR & 1e-3 \\
         & Llama &  &  &  &  & WCA & 1e-4\\ 
         & Mamba &  &  &  &  & WCA & 1e-3\\ 
         & LSTM &  &  &  &  & X & X\\ 
         & RWKV-4 &  &  &  &  & WCAR & 1e-3\\
         & LSTM-SM &  &  &  &  & WCA & 1e-3\\ 
         & xLSTM[1:0] &  &  &  &  & WCAR & 1e-3 \\ 
    \midrule
        \multirow{9}{*}{ListOps} & Transformer & \multirow{9}{*}{8} & \multirow{9}{*}{128} & \multirow{9}{*}{32} & \multirow{9}{*}{80K} & WCA & 1e-4 \\ 
         & Llama &  &  &  &  & WCA & 1e-4\\ 
         & Mamba &  &  &  &  & WCA & 1e-3\\ 
         & LSTM &  &  &  &  & WCA & 1e-3\\ 
         & RWKV-4 &  &  &  &  & WCA & 6e-4\\ 
         & LSTM-SM &  &  &  &  & WCA & 1e-3\\ 
         & xLSTM[1:0] &  &  &  &  & WCA & 1e-3 \\ 
    \midrule
        \multirow{9}{*}{Pathfinder} & Transformer & \multirow{9}{*}{6} & \multirow{9}{*}{192} & \multirow{9}{*}{64} & \multirow{9}{*}{500K} & WCAR & 1e-4 \\ 
         & Llama &  &  &  &  & WCAR & 1e-4\\ 
         & Mamba &  &  &  &  & WCA & 1e-3\\ 
         & LSTM &  &  &  &  & X & X\\ 
         & RWKV-4 &  &  &  &  & WCA & 1e-4\\ 
         & LSTM-SM &  &  &  &  & X & X\\ 
         & xLSTM[1:0] &  &  &  &  & WCA & 1e-4 \\ 
    \midrule
        \multirow{9}{1.3cm}{G-Image} & Transformer & \multirow{9}{*}{6} & \multirow{9}{*}{512} & \multirow{9}{*}{64} & \multirow{9}{*}{180K} & WCAR & 6e-4 \\ 
         & Llama &  &  &  &  & WCAR & 6e-4\\ 
         & Mamba &  &  &  &  & WCA & 6e-4\\ 
         & LSTM &  &  &  &  & WCAR & 1e-3\\ 
         & LSTM &  &  &  &  & WCAR & 1e-3\\ 
         & RWKV-4 &  &  &  &  & WCA & 1e-3\\ 
         & LSTM-SM &  &  &  &  & WCA & 6e-4\\ 
         & xLSTM[0:1] &  &  &  &  & WCAR & 1e-3\\ 
    \midrule
        \multirow{9}{1.3cm}{RGB-Image} & Transformer & \multirow{9}{*}{6} & \multirow{9}{*}{512} & \multirow{9}{*}{64} & \multirow{9}{*}{180K} & WCA & 6e-4 \\ 
         & Llama &  &  &  &  & WCAR & 1e-4\\ 
         & Mamba &  &  &  &  & WCAR & 1e-3\\ 
         & LSTM &  &  &  &  & WCAR & 1e-3\\ 
         & RWKV-4 &  &  &  &  & WCAR & 6e-4\\ 
         & LSTM-SM &  &  &  &  & WCA & 6e-4\\ 
         & xLSTM[0:1] &  &  &  &  & WCAR & 1e-3\\        
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{List detailing all the hyperparameters used in each of the Long Range Arena benchmark. "X" denotes models which fail to outperform the random baseline. \JB{Not sure if we need this table at all} 
    %\GK{remove vertical lines to fit style of other tables}
    }
    \label{tab:lra_hyperparameters}
\end{table}

==> tables/lra_val_accuracy.tex <==
\begin{table}
    \centering
    \begin{adjustbox}{width=1.0\textwidth}
    \begin{tabular}{lcccccc}
    \toprule
    & \textbf{Retrieval} & \textbf{ListOps} & \textbf{Pathfinder} & \textbf{G-Image} & \textbf{RGB-Image} & \textbf{Ranking} \\ \midrule
Random Baseline & 0.500 & 0.100 & 0.500 & 0.100 & 0.100 &  \\ \midrule
Transformer & 0.834 & 0.415 & 0.848 & 0.537 & 0.655 & 6 \\ 
Llama & 0.859 & 0.583 & 0.833 & 0.551 & 0.647 & 5\\ \midrule
Mamba & 0.911 & \underline{0.599} & \textbf{0.970} & 0.740 & \textbf{0.828} & 2 \\ \midrule
LSTM & X & 0.377 & X & 0.721 & 0.754 & 6 \\ 
RWKV-4 & \underline{0.912} & 0.595 & 0.885 & 0.726 & 0.804 & 3\\ 
LSTM-SM & 0.887 & 0.546 & X & \underline{0.741} & 0.804 & 4 \\ \midrule
xLSTM & \textbf{0.915} & \textbf{0.623} & \underline{0.912} & \textbf{0.751} & \underline{0.816} & 1 \\ 
\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Long Range Arena validation tasks. Bold highlights the best performing model, underlined the second best. X denotes models that fail to outperform random baselines.
    \GK{
    %removed the vertical lines to fit style of other tables; 
    smaller other formatting changes}
    }
    \label{tab:lra_val_accuracy}
    
\end{table}

==> tables/lra_xlstm_hyperparameters.tex <==
\begin{table}
    \centering
    \begin{tabular}{lcccccc}
    \toprule
    & \textbf{Retrieval} & \textbf{ListOps} & \textbf{Pathfinder} & \textbf{G-Image} & \textbf{RGB-Image} \\ 
    \midrule
sLSTM Number of Blocks & 0 & 0 & 0 & 6 & 6  \\ 
mLSTM Number of Blocks & 6 & 8 & 6 & 0 & 0 \\ 
\bottomrule
    \end{tabular}
    \caption{Architecture of xLSTM model for Long Range Arena tasks. \JB{Also not needed I guess? I will put the block ratio in the xLSTM name in the next table.} \GK{could be just put in the text.}}
    \label{tab:lra_xlstm_hyperparameters}
\end{table}

==> tables/raw_spaj15b_res_test_abl2.tex <==
\begin{tabular}{llrr}
\toprule
A & run_name_disamb & num_model_params & _Perplexity-train_step-best \\
\midrule
0 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1noconv_0-B48E1024H4gbs256 & 408 & 13.88 \\
1 & spaj15b-xlstmblock2-350M_vlstmv2_abl_fgateigbiasonly_0-B48E1024H4gbs256 & 409 & 13.88 \\
2 & spaj15b-xlstmblock2-350M_xlstmv2_fprodv0_0-B48E1024H4gbs256 & 408 & 13.82 \\
3 & spaj15b-xlstmblock2-350M_vlstmv2_abl_fgdecay_0-B48E1024H4gbs256 & 409 & 14.09 \\
4 & spaj15b-xlstmblock2-350M_vlstmv2_abl_noconvnocact_0-B48E1024H4gbs256 & 409 & 15.77 \\
5 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv2_2-B48E1024H4gbs256 & 410 & 13.97 \\
6 & spaj15b-xlstmblock2P-350M_slstmv2p_fprodv0_4-B48E1024H4gbs256 & 405 & 22.43 \\
7 & spaj15b-xlstmblock2-350M_vlstmv2_abl_igonlyfgdecinit_0-B48E1024H4gbs256 & 409 & 14.03 \\
8 & spaj15b-xlstmblock2-350M_vlstmv2_abl_fgonly_0-B48E1024H4gbs256 & 409 & 13.90 \\
9 & spaj15b-xlstmblock2-350M_slstmv2_fprodv0_2-B48E1024H4gbs256 & 418 & 17.28 \\
10 & spaj15b-vlstm-350M_vlstmv1_fprodv0_0-B24E1024H4gbs256 & 430 & 14.24 \\
11 & spaj15b-xlstmblock2-350M_slstmv2seed42_fprodv0_0-B48E1024H4gbs256 & 418 & 17.11 \\
12 & spaj15b-xlstmblock2-125M_vlstmv2_fprodv0_0-B24E768H4gbs256 & 164 & 16.55 \\
13 & spaj15b-xlstmblock2-350M_vlstmv2_fprodv0_0-B48E1024H4gbs256 & 409 & 13.77 \\
14 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_2-B48E1024H4gbs256 & 402 & 18.35 \\
15 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_3-B48E1024H4gbs256 & 402 & 18.44 \\
16 & spaj15b-xlstmblock2U-350M_slstmv2u_fprodv0_3-B48E1024H4gbs256 & 406 & 19.20 \\
17 & spaj15b-xlstmblock2-350M_vlstmv2_abl_nogatesfgdecinit_0-B48E1024H4gbs256 & 409 & 14.28 \\
18 & spaj15b-xlstmblock2-350M_vlstmv2_abl_fgdecayigbiasonly_0-B48E1024H4gbs256 & 409 & 14.06 \\
19 & spaj15b-xlstmblock2P-350M_slstmv1noconvact_fprodv0_0-B24E1024H4gbs256 & 427 & 17.38 \\
20 & spaj15b-xlstmblock2P-350M_slstmv1noconvact_fprodv0_0-B48E1024H4gbs256 & 402 & 17.95 \\
21 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[0, 1, 2, 3, 4, 5] & 408 & 13.84 \\
22 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[19, 21, 23, 25, 27, 29] & 408 & 14.10 \\
23 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[1, 3, 5, 42, 44, 46] & 408 & 13.77 \\
24 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[21, 22, 23, 24, 25, 26] & 408 & 14.07 \\
25 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[3, 11, 19, 27, 35, 43] & 408 & 13.94 \\
26 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2ratio_0-B48E1024H4gbs256_slstm_ffbl_loc[5, 42] & 409 & 13.77 \\
27 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2ratio_0-B48E1024H4gbs256_slstm_ffbl_loc[3, 5, 7, 9, 38, 40, 42, 44] & 408 & 13.96 \\
28 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2ratio_0-B48E1024H4gbs256_slstm_ffbl_loc[3, 5, 42, 44] & 409 & 13.81 \\
29 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_0-B24E1024H4gbs256_kernel_size0.0 & 427 & 17.74 \\
30 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_0-B24E1024H4gbs256_kernel_size4.0 & 427 & 17.95 \\
\bottomrule

\caption{xLSTM Model Ablations Test PPL}
\end{tabular}


==> tables/raw_spaj15b_res_test_models.tex <==
\begin{tabular}{llrr}
\toprule
 & run_name_disamb & num_model_params & _Perplexity-train_step-best \\
\midrule
0 & spaj15b-xlstmblock2P-350M_slstmv2p_fprodv0_4-B48E1024H4gbs256 & 405 & 22.43 \\
1 & spaj15b-rwkv4_lm-350M_rwkv4_fprodv1_0-B24E1024H0gbs256 & 430 & 15.87 \\
2 & spaj15b-customselfattention-350M_llama_fprodv0_1-B24E1024H16gbs256 & 407 & 14.64 \\
3 & spaj15b-xlstmblock2U-350M_slstmv2u_fprodv0_3-B48E1024H4gbs256 & 406 & 19.20 \\
4 & spaj15b-xlstmblock2-350M_slstmv2seed42_fprodv0_0-B48E1024H4gbs256 & 418 & 17.11 \\
5 & spaj15b-lstm-350M_lstmseqmix_fprodv0_0-B24E1024H0gbs256 & 506 & 26.41 \\
6 & spaj15b-rwkv5_lm-350M_rwkv5_fprodv1_0-B24E1024H0gbs256 & 456 & 16.88 \\
7 & spaj15b-rwkv5_lm-350M_rwkv5wd_fprodv2_1-B24E1024H0gbs256 & 456 & 16.93 \\
8 & spaj15b-h3_lm-350M_h3_fprodv0_0-B48E1024H0gbs256 & 420 & 18.48 \\
9 & spaj15b-mamba-350M_mamba_fprodv1_0-B48E1024H0gbs256 & 423 & 14.38 \\
10 & spaj15b-vlstm-350M_vlstmv1_fprodv0_0-B24E1024H4gbs256 & 430 & 14.24 \\
11 & spaj15b-transformer_lm-350M_retention_fprodv1_0-B24E1024H0gbs256 & 431 & 16.52 \\
12 & spaj15b-transformer_lm-350M_retention_fprodv0_1-B48E1024H0gbs256 & 758 & 14.93 \\
13 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_2-B48E1024H4gbs256 & 402 & 18.35 \\
14 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_3-B48E1024H4gbs256 & 402 & 18.44 \\
15 & spaj15b-rwkv5_lm-350M_rwkv5_fprodv0_0-B48E1024H0gbs256 & 808 & 16.08 \\
16 & spaj15b-xlstmblock2P-350M_slstmv1noconvact_fprodv0_0-B24E1024H4gbs256 & 427 & 17.38 \\
17 & spaj15b-xlstmblock2P-350M_slstmv1noconvact_fprodv0_0-B48E1024H4gbs256 & 402 & 17.95 \\
18 & spaj15b-hyena_lm-350M_hyena_fprodv0_0-B48E1024H0gbs256 & 435 & 17.85 \\
19 & spaj15b-transformer_lm-350Mde_lstmmultilayerblock_fprodv0_0-B48E1024H0gbs256 & 506 & 35.95 \\
20 & spaj15b-transformer_lm-350Mwi_lstmmultilayerblock_fprodv0_0-B24E1536H0gbs256 & 608 & 30.69 \\
21 & spaj15b-xlstmblock2-350M_slstmv2_fprodv0_2-B48E1024H4gbs256 & 418 & 17.28 \\
22 & spaj15b-xlstmblock2-350M_xlstmv2_fprodv0_0-B48E1024H4gbs256 & 408 & 13.82 \\
23 & spaj15b-lstm_lm-350Mwi_lstmmultilayer_fprodv0_0-B24E1536H0gbs256 & 608 & 2424.11 \\
24 & spaj15b-xlstmblock2-125M_vlstmv2_fprodv0_0-B24E768H4gbs256 & 164 & 16.55 \\
25 & spaj15b-xlstmblock2-350M_vlstmv2_fprodv0_0-B48E1024H4gbs256 & 409 & 13.77 \\
26 & spaj15b-rwkv5_lm-350M_rwkv5wd_fprodv0_0-B48E1024H0gbs256 & 808 & 16.05 \\
27 & spaj15b-rwkv6_lm-350M_rwkv6_fprodv0_0-B24E1024H0gbs256 & 442 & 17.83 \\
28 & spaj15b-customselfattention-350M_gpt_fprodv0_0-B24E1024H16gbs256_lr0.0003 & 356 & 16.53 \\
29 & spaj15b-mamba-350M_mamba_fprodv0_0-B48E1024H0gbs256_tie_weightsFalse & 423 & 14.01 \\
30 & spaj15b-mamba-350M_mamba_fprodv0_0-B48E1024H0gbs256_tie_weightsTrue & 372 & 14.03 \\
31 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_0-B24E1024H4gbs256_kernel_size0.0 & 427 & 17.74 \\
32 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_0-B24E1024H4gbs256_kernel_size4.0 & 427 & 17.95 \\
33 & spaj15b-customselfattention-350M_gpt_fprodv0_0-B24E1024H16gbs256_precision_pos_emb_adddefault & 356 & 14.65 \\
34 & spaj15b-customselfattention-350M_gpt_fprodv0_0-B24E1024H16gbs256_precision_pos_emb_addfloat32 & 356 & 14.68 \\
35 & GLA & 412& 20.04 \\
36 & HGRN2 & 411& 17.15 \\
37 & HGRN & 411 & 22.09\\
\bottomrule
\caption{xLSTM Benchmark Models Test PPL}
\end{tabular}


==> tables/raw_spaj15b_res_val_abl2.tex <==
\begin{tabular}{llrr}
\toprule
 & run_name_disamb & num_model_params & _Perplexity-train_step-best \\
\midrule
0 & spaj15b-xlstmblock2-350M_vlstmv2_abl_igonlyfgdecinit_0-B48E1024H4gbs256 & 409 & 13.68 \\
1 & spaj15b-xlstmblock2-350M_vlstmv2_abl_fgonly_0-B48E1024H4gbs256 & 409 & 13.56 \\
2 & spaj15b-xlstmblock2-350M_slstmv2_fprodv0_2-B48E1024H4gbs256 & 418 & 16.99 \\
3 & spaj15b-xlstmblock2-350M_vlstmv2_abl_fgdecay_0-B48E1024H4gbs256 & 409 & 13.74 \\
4 & spaj15b-xlstmblock2-350M_vlstmv2_abl_fgdecayigbiasonly_0-B48E1024H4gbs256 & 409 & 13.71 \\
5 & spaj15b-xlstmblock2-350M_vlstmv2_abl_nogatesfgdecinit_0-B48E1024H4gbs256 & 409 & 13.94 \\
6 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv2_2-B48E1024H4gbs256 & 410 & 13.62 \\
7 & spaj15b-vlstm-350M_vlstmv1_fprodv0_0-B24E1024H4gbs256 & 430 & 13.89 \\
8 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1noconv_0-B48E1024H4gbs256 & 408 & 13.54 \\
9 & spaj15b-xlstmblock2-350M_vlstmv2_abl_fgateigbiasonly_0-B48E1024H4gbs256 & 409 & 13.54 \\
10 & spaj15b-xlstmblock2-125M_vlstmv2_fprodv0_0-B24E768H4gbs256 & 164 & 16.12 \\
11 & spaj15b-xlstmblock2-350M_vlstmv2_fprodv0_0-B48E1024H4gbs256 & 409 & 13.43 \\
12 & spaj15b-xlstmblock2-350M_xlstmv2_fprodv0_0-B48E1024H4gbs256 & 408 & 13.48 \\
13 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_2-B48E1024H4gbs256 & 402 & 18.08 \\
14 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_3-B48E1024H4gbs256 & 402 & 18.18 \\
15 & spaj15b-xlstmblock2U-350M_slstmv2u_fprodv0_3-B48E1024H4gbs256 & 406 & 18.86 \\
16 & spaj15b-xlstmblock2P-350M_slstmv1noconvact_fprodv0_0-B24E1024H4gbs256 & 427 & 17.14 \\
17 & spaj15b-xlstmblock2P-350M_slstmv1noconvact_fprodv0_0-B48E1024H4gbs256 & 402 & 17.70 \\
18 & spaj15b-xlstmblock2-350M_vlstmv2_abl_noconvnocact_0-B48E1024H4gbs256 & 409 & 15.39 \\
19 & spaj15b-xlstmblock2P-350M_slstmv2p_fprodv0_4-B48E1024H4gbs256 & 405 & 22.08 \\
20 & spaj15b-xlstmblock2-350M_slstmv2seed42_fprodv0_0-B48E1024H4gbs256 & 418 & 16.82 \\
21 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[0, 1, 2, 3, 4, 5] & 408 & 13.50 \\
22 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[19, 21, 23, 25, 27, 29] & 408 & 13.75 \\
23 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[1, 3, 5, 42, 44, 46] & 408 & 13.43 \\
24 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[21, 22, 23, 24, 25, 26] & 408 & 13.71 \\
25 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2pos_0-B48E1024H4gbs256_slstm_ffbl_loc[3, 11, 19, 27, 35, 43] & 408 & 13.60 \\
26 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2ratio_0-B48E1024H4gbs256_slstm_ffbl_loc[3, 5, 7, 9, 38, 40, 42, 44] & 408 & 13.62 \\
27 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2ratio_0-B48E1024H4gbs256_slstm_ffbl_loc[5, 42] & 409 & 13.43 \\
28 & spaj15b-xlstmblock2-350M_xlstmv2_abl_sv1mv2ratio_0-B48E1024H4gbs256_slstm_ffbl_loc[3, 5, 42, 44] & 409 & 13.47 \\
29 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_0-B24E1024H4gbs256_kernel_size0.0 & 427 & 17.49 \\
30 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_0-B24E1024H4gbs256_kernel_size4.0 & 427 & 17.68 \\
\bottomrule
\caption{xLSTM Model Ablations Val PPL}
\end{tabular}


==> tables/raw_spaj15b_res_val_models.tex <==
\begin{tabular}{llrr}
\toprule
 & run_name_disamb & num_model_params & _Perplexity-train_step-best \\
\midrule
0 & spaj15b-xlstmblock2-350M_slstmv2seed42_fprodv0_0-B48E1024H4gbs256 & 418 & 16.82 \\
1 & spaj15b-rwkv6_lm-350M_rwkv6_fprodv0_0-B24E1024H0gbs256 & 442 & 17.40 \\
2 & spaj15b-xlstmblock2U-350M_slstmv2u_fprodv0_3-B48E1024H4gbs256 & 406 & 18.86 \\
3 & spaj15b-h3_lm-350M_h3_fprodv0_0-B48E1024H0gbs256 & 420 & 18.23 \\
4 & spaj15b-transformer_lm-350M_retention_fprodv0_1-B48E1024H0gbs256 & 758 & 14.59 \\
5 & spaj15b-rwkv5_lm-350M_rwkv5wd_fprodv2_1-B24E1024H0gbs256 & 456 & 16.58 \\
6 & spaj15b-rwkv5_lm-350M_rwkv5_fprodv0_0-B48E1024H0gbs256 & 808 & 15.75 \\
7 & spaj15b-vlstm-350M_vlstmv1_fprodv0_0-B24E1024H4gbs256 & 430 & 13.89 \\
8 & spaj15b-lstm-350M_lstmseqmix_fprodv0_0-B24E1024H0gbs256 & 506 & 26.07 \\
9 & spaj15b-rwkv5_lm-350M_rwkv5wd_fprodv0_0-B48E1024H0gbs256 & 808 & 15.71 \\
10 & spaj15b-xlstmblock2-350M_slstmv2_fprodv0_2-B48E1024H4gbs256 & 418 & 16.99 \\
11 & spaj15b-lstm_lm-350Mwi_lstmmultilayer_fprodv0_0-B24E1536H0gbs256 & 608 & 2417.88 \\
12 & spaj15b-rwkv5_lm-350M_rwkv5_fprodv1_0-B24E1024H0gbs256 & 456 & 16.53 \\
13 & spaj15b-transformer_lm-350M_retention_fprodv1_0-B24E1024H0gbs256 & 431 & 16.23 \\
14 & spaj15b-transformer_lm-350Mde_lstmmultilayerblock_fprodv0_0-B48E1024H0gbs256 & 506 & 35.45 \\
15 & spaj15b-transformer_lm-350Mwi_lstmmultilayerblock_fprodv0_0-B24E1536H0gbs256 & 608 & 30.28 \\
16 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_2-B48E1024H4gbs256 & 402 & 18.08 \\
17 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_3-B48E1024H4gbs256 & 402 & 18.18 \\
18 & spaj15b-xlstmblock2-125M_vlstmv2_fprodv0_0-B24E768H4gbs256 & 164 & 16.12 \\
19 & spaj15b-xlstmblock2-350M_vlstmv2_fprodv0_0-B48E1024H4gbs256 & 409 & 13.43 \\
20 & spaj15b-xlstmblock2P-350M_slstmv2p_fprodv0_4-B48E1024H4gbs256 & 405 & 22.08 \\
21 & spaj15b-xlstmblock2P-350M_slstmv1noconvact_fprodv0_0-B24E1024H4gbs256 & 427 & 17.14 \\
22 & spaj15b-xlstmblock2P-350M_slstmv1noconvact_fprodv0_0-B48E1024H4gbs256 & 402 & 17.70 \\
23 & spaj15b-customselfattention-350M_llama_fprodv0_1-B24E1024H16gbs256 & 407 & 14.25 \\
24 & spaj15b-xlstmblock2-350M_xlstmv2_fprodv0_0-B48E1024H4gbs256 & 408 & 13.48 \\
25 & spaj15b-mamba-350M_mamba_fprodv1_0-B48E1024H0gbs256 & 423 & 14.06 \\
26 & spaj15b-hyena_lm-350M_hyena_fprodv0_0-B48E1024H0gbs256 & 435 & 17.59 \\
27 & spaj15b-rwkv4_lm-350M_rwkv4_fprodv1_0-B24E1024H0gbs256 & 430 & 15.62 \\
28 & spaj15b-customselfattention-350M_gpt_fprodv0_0-B24E1024H16gbs256_lr0.0003 & 356 & 16.08 \\
29 & spaj15b-mamba-350M_mamba_fprodv0_0-B48E1024H0gbs256_tie_weightsFalse & 423 & 13.70 \\
30 & spaj15b-mamba-350M_mamba_fprodv0_0-B48E1024H0gbs256_tie_weightsTrue & 372 & 13.71 \\
31 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_0-B24E1024H4gbs256_kernel_size0.0 & 427 & 17.49 \\
32 & spaj15b-xlstmblock2P-350M_slstmv1_fprodv0_0-B24E1024H4gbs256_kernel_size4.0 & 427 & 17.68 \\
33 & spaj15b-customselfattention-350M_gpt_fprodv0_0-B24E1024H16gbs256_precision_pos_emb_adddefault & 356 & 14.26 \\
34 & spaj15b-customselfattention-350M_gpt_fprodv0_0-B24E1024H16gbs256_precision_pos_emb_addfloat32 & 356 & 14.29 \\
35 & GLA & 412& 19.56
36 & HGRN2 & 411& 16.77
37 & HGRN & 411 & 21.83
\bottomrule
\caption{xLSTM Benchmark Models Val PPL}
\end{tabular}

